Recursive Decomposition of Logical Thoughts: Framework for Superior Reasoning and Knowledge Propagation in Large Language Models

Enhancing the reasoning capabilities of Large Language Models remains a critical challenge in artificial intelligence. We introduce RDoLT, Recursive Decomposition of Logical Thought prompting, a novel framework that significantly boosts LLM reasoning performance. RDoLT is built on three key innovations: (1) recursively breaking down complex reasoning tasks into sub-tasks of progressive complexity; (2) employing an advanced selection and scoring mechanism to identify the most promising reasoning thoughts; and (3) integrating a knowledge propagation module that mimics human learning by keeping track of strong and weak thoughts for information propagation. Our approach was evaluated across multiple benchmarks, including GSM8K, SVAMP, MultiArith, LastLetterConcatenation, and Gaokao2023 Math. The results demonstrate that RDoLT consistently outperforms existing state-of-the-art techniques, achieving a 90.98 percent accuracy on GSM8K with ChatGPT-4, surpassing state-of-the-art techniques by 6.28 percent. Similar improvements were observed on other benchmarks, with accuracy gains ranging from 5.5 percent to 6.75 percent. These findings highlight RDoLT's potential to advance prompt engineering, offering a more effective and generalizable approach to complex reasoning tasks.

==> corrected_bibliography.tex <==
\begin{thebibliography}{99}
  \bibitem{information_retrieval_llms}
    Kitab: Evaluating llms on constraint satisfaction for information retrieval. 2023.

  \bibitem{inforRetmeetLLMs}
    {Information Retrieval meets Large Language Models: A strategic report from Chinese IR community. 2023.

  \bibitem{llama3modelcard}
    Llama 3 Model Card. 2024.

  \bibitem{qwen2}
    Qwen2 Technical Report. 2024.

  \bibitem{reinforcmentfromhumanfeedback}
    Training a Helpful and Harmless Assistant with Reinforcement Learning from Human Feedback. 2022.

  \bibitem{graph_of_thoughts_solving_elaborate_problems_with_large_language_models}
    Graph of Thoughts: Solving Elaborate Problems with Large Language Models. 2024.

  \bibitem{topologies_of_reasoning_demystifying_chains_trees_and_graphs_of_thoughts}
    Topologies of Reasoning: Demystifying Chains, Trees, and Graphs of Thoughts. 2024.

  \bibitem{Q&A}
    Cross-Data Knowledge Graph Construction for LLM-enabled Educational Question-Answering System: A Case Study at HCMUT. 2024.

  \bibitem{chen2024inside}
    INSIDE: LLMs' Internal States Retain the Power of Hallucination Detection. 2024.

  \bibitem{chen2023teachinglargelanguagemodels}
    Teaching Large Language Models to Self-Debug. 2023.

  \bibitem{LastLetterConcat}
    {ChilleD/LastLetterConcat · Datasets at Hugging Face. 2023.

  \bibitem{MultiArith}
    {ChilleD/MultiArith · Datasets at Hugging Face. 2023.

  \bibitem{chain-of-thought_prompting_elicits_reasoning_in_large_language_models}
    ChilleD/LastLetterConcat · Datasets at Hugging Face. 2023.

  \bibitem{gmsk8}
    Training Verifiers to Solve Math Word Problems. 2021.

  \bibitem{llm_task_planning}
    Integrating action knowledge and LLMs for task planning and situation handling in open worlds. 2023.

  \bibitem{NL-Edit}
    NL-EDIT: Correcting semantic parse errors through natural language interaction. 2021.

  \bibitem{erdem2022neural}
    Neural natural language generation: A survey on multilinguality, multimodality, controllability and learning. 2022.

  \bibitem{llm_based_machine_translation_for_ecommerce}
    LLMs-based machine translation for E-commerce. 2024.

  \bibitem{large_language_models_are_not_strong_abstract_reasoners}
    Large Language Models Are Not Strong Abstract Reasoners. 2023.

  \bibitem{llm_and_Ai_reach_and_impact}
    Llms and ai: Understanding its reach and impact. 2023.

  \bibitem{abstraction_of_thought_makes_language_models_better_reasoners}
    Abstraction-of-Thought Makes Language Models Better Reasoners. 2024.

  \bibitem{large_language_models_cannot_self_correct_reasoning_yet}
    Large Language Models Cannot Self-Correct Reasoning Yet. 2023.

  \bibitem{NEURIPS2022_8636419d}
    CodeRL: Mastering Code Generation through Pretrained Models and Deep Reinforcement Learning. 2022.

  \bibitem{Question-Asking_LLMs}
    MEDIQ: Question-Asking LLMs for Adaptive and Reliable Medical Reasoning. 2024.

  \bibitem{lin-etal-2020-commongen}
    {C. 2020.

  \bibitem{RainierReinforcedKnowledgeIntrospector}
    Rainier: Reinforced Knowledge Introspector for Commonsense Question Answering. 2022.

  \bibitem{llm_as_A_testing_expert-gui_testing}
    Make llm a testing expert: Bringing human-like interaction to mobile gui testing via functionality-aware decisions. 2024.

  \bibitem{NEURIPS2022_b125999b}
    QUARK: Controllable Text Generation with Reinforced Unlearning. 2022.

  \bibitem{madaan2023selfrefineiterativerefinementselffeedback}
    Self-Refine: Iterative Refinement with Self-Feedback. 2023.

  \bibitem{agent_llms}
    LLM-Powered Conversational Voice Assistants: Interaction Patterns, Opportunities, Challenges, and Design Guidelines. 2023.

  \bibitem{mirowski2022cowritingscreenplaystheatrescripts}
    Co-Writing Screenplays and Theatre Scripts with Language Models: An Evaluation by Industry Professionals. 2022.

  \bibitem{llm_fun_challenges_opp_and_social_impact}
    Foundation and large language models: fundamentals, challenges, opportunities, and social impacts. 2024.

  \bibitem{ollama}
    {Ollama: Get up and running with Llama 3.1, Mistral, Gemma 2, and other large language models. 2024.

  \bibitem{openai2024gpt4technicalreport}
    GPT-4 Technical Report. 2024.

  \bibitem{can_separators_improve_chain_of_thought_prompting_}
    Can Separators Improve Chain-of-Thought Prompting?. 2024.

  \bibitem{patel-etal-2021-nlp}
    Are {NLP. 2021.

  \bibitem{paul2024refinerreasoningfeedbackintermediate}
    REFINER: Reasoning Feedback on Intermediate Representations. 2024.

  \bibitem{lm_studio_-_discover_download_and_run_local_llms}
    Machine Translation with Large Language Models: Prompt Engineering for Persian, English, and Russian Directions. 2024.

  \bibitem{can_github_issues_be_solved_with_tree_of_thoughts_}
    Can Github issues be solved with Tree Of Thoughts?. 2024.

  \bibitem{can_llm_master_math_no}
    Can LLMs Master Math? Investigating Large Language Models on Math Stack Exchange. 2024.

  \bibitem{algorithm_of_thoughts_enhancing_exploration_of_ideas_in_large_language_models}
    Algorithm of Thoughts: Enhancing Exploration of Ideas in Large Language Models. 2023.

  \bibitem{small_llms_are_weak_tool_learners_a_multi_llm_agent}
    Small LLMs Are Weak Tool Learners: A Multi-LLM Agent. 2024.

  \bibitem{shinn2023reflexionlanguageagentsverbal}
    Reflexion: Language Agents with Verbal Reinforcement Learning. 2023.

  \bibitem{chain_of_thoughtlessness}
    Chain of Thoughtlessness? An Analysis of CoT in Planning. 2024.

  \bibitem{learntorepair}
    {Learning to Repair: Repairing model output errors after deployment using a dynamic memory of feedback. 2021.

  \bibitem{gemma_2024}
    Gemma. 2024.

  \bibitem{LLMs_generate_human-like_opinions}
    ChatGPT as a commenter to the news: can LLMs generate human-like opinions?. 2023.

  \bibitem{van2024hybrid}
    A hybrid intelligence method for argument mining. 2024.

  \bibitem{vatsal2024surveypromptengineeringmethods}
    A Survey of Prompt Engineering Methods in Large Language Models for Different NLP Tasks. 2024.

  \bibitem{self_consistency_improves_chain_of_thought_reasoning_in_language_models}
    Self-Consistency Improves Chain of Thought Reasoning in Language Models. 2022.

  \bibitem{wang2024describeexplainplanselect}
    Describe, Explain, Plan and Select: Interactive Planning with Large Language Models Enables Open-World Multi-Task Agents. 2024.

  \bibitem{chain_of_thought_prompting_elicits_reasoning_in_large_language_models}
    Chain-of-Thought Prompting Elicits Reasoning in Large Language Models. 2022.

  \bibitem{welleck2022generatingsequenceslearningselfcorrect}
    Generating Sequences by Learning to Self-Correct. 2022.

  \bibitem{decomosition_of_task_with_llms}
    MLDT: Multi-Level Decomposition for Complex Long-Horizon Robotic Task Planning with Open-Source Large Language Model. 2024.

  \bibitem{xie2023selfevaluationguidedbeamsearch}
    Self-Evaluation Guided Beam Search for Reasoning. 2023.

  \bibitem{xing2024designing}
    Designing heterogeneous llm agents for financial sentiment analysis. 2024.

  \bibitem{unlocking_the_potential_a_comprehensive_exploration_of_large_language_models_in_natural_language_processing}
    Unlocking the potential: A comprehensive exploration of large language models in natural language processing. 2024.

  \bibitem{generative_ai_in_the_era_of_transformers_revolutionizing_natural_language_processing_with_llms}
    Generative AI in the Era of Transformers: Revolutionizing Natural Language Processing with LLMs. 2024.

  \bibitem{large_language_models_are_contrastive_reasoners}
    Large Language Models are Contrastive Reasoners. 2024.

  \bibitem{tree_of_thoughts_deliberate_problem_solving_with_large_language_models}
    Tree of Thoughts: Deliberate Problem Solving with Large Language Models. 2023.

  \bibitem{yao2023reactsynergizingreasoningacting}
    ReAct: Synergizing Reasoning and Acting in Language Models. 2023.

  \bibitem{llm_healthcare}
    Leveraging generative AI and large Language models: a Comprehensive Roadmap for Healthcare Integration. 2023.

  \bibitem{text_Summary}
    A Systematic Survey of Text Summarization: From Statistical Methods to Large Language Models. 2024.

  \bibitem{zhang2023exploring}
    Exploring collaboration mechanisms for llm agents: A social psychology view. 2023.

  \bibitem{gaokao-math}
    Evaluating the Performance of Large Language Models on GAOKAO Benchmark. 2023.

  \bibitem{zhou2024misinformingllmsvulnerabilitieschallenges}
    Misinforming LLMs: vulnerabilities, challenges and opportunities. 2024.

  \bibitem{least_to_most_prompting_enables_complex_reasoning_in_large_language_models}
    Least-to-Most Prompting Enables Complex Reasoning in Large Language Models. 2022.

  \bibitem{information_retrieval_llms}
    Kitab: Evaluating llms on constraint satisfaction for information retrieval. 2023.

  \bibitem{inforRetmeetLLMs}
    {Information Retrieval meets Large Language Models: A strategic report from Chinese IR community. 2023.

  \bibitem{llama3modelcard}
    Llama 3 Model Card. 2024.

  \bibitem{qwen2}
    Qwen2 Technical Report. 2024.

  \bibitem{reinforcmentfromhumanfeedback}
    Training a Helpful and Harmless Assistant with Reinforcement Learning from Human Feedback. 2022.

  \bibitem{graph_of_thoughts_solving_elaborate_problems_with_large_language_models}
    Graph of Thoughts: Solving Elaborate Problems with Large Language Models. 2024.

  \bibitem{topologies_of_reasoning_demystifying_chains_trees_and_graphs_of_thoughts}
    Topologies of Reasoning: Demystifying Chains, Trees, and Graphs of Thoughts. 2024.

  \bibitem{Q&A}
    Cross-Data Knowledge Graph Construction for LLM-enabled Educational Question-Answering System: A Case Study at HCMUT. 2024.

  \bibitem{chen2024inside}
    INSIDE: LLMs' Internal States Retain the Power of Hallucination Detection. 2024.

  \bibitem{chen2023teachinglargelanguagemodels}
    Teaching Large Language Models to Self-Debug. 2023.

  \bibitem{LastLetterConcat}
    {ChilleD/LastLetterConcat · Datasets at Hugging Face. 2023.

  \bibitem{MultiArith}
    {ChilleD/MultiArith · Datasets at Hugging Face. 2023.

  \bibitem{chain-of-thought_prompting_elicits_reasoning_in_large_language_models}
    ChilleD/LastLetterConcat · Datasets at Hugging Face. 2023.

  \bibitem{gmsk8}
    Training Verifiers to Solve Math Word Problems. 2021.

  \bibitem{llm_task_planning}
    Integrating action knowledge and LLMs for task planning and situation handling in open worlds. 2023.

  \bibitem{NL-Edit}
    NL-EDIT: Correcting semantic parse errors through natural language interaction. 2021.

  \bibitem{erdem2022neural}
    Neural natural language generation: A survey on multilinguality, multimodality, controllability and learning. 2022.

  \bibitem{llm_based_machine_translation_for_ecommerce}
    LLMs-based machine translation for E-commerce. 2024.

  \bibitem{large_language_models_are_not_strong_abstract_reasoners}
    Large Language Models Are Not Strong Abstract Reasoners. 2023.

  \bibitem{llm_and_Ai_reach_and_impact}
    Llms and ai: Understanding its reach and impact. 2023.

  \bibitem{abstraction_of_thought_makes_language_models_better_reasoners}
    Abstraction-of-Thought Makes Language Models Better Reasoners. 2024.

  \bibitem{large_language_models_cannot_self_correct_reasoning_yet}
    Large Language Models Cannot Self-Correct Reasoning Yet. 2023.

  \bibitem{NEURIPS2022_8636419d}
    CodeRL: Mastering Code Generation through Pretrained Models and Deep Reinforcement Learning. 2022.

  \bibitem{Question-Asking_LLMs}
    MEDIQ: Question-Asking LLMs for Adaptive and Reliable Medical Reasoning. 2024.

  \bibitem{lin-etal-2020-commongen}
    {C. 2020.

  \bibitem{RainierReinforcedKnowledgeIntrospector}
    Rainier: Reinforced Knowledge Introspector for Commonsense Question Answering. 2022.

  \bibitem{llm_as_A_testing_expert-gui_testing}
    Make llm a testing expert: Bringing human-like interaction to mobile gui testing via functionality-aware decisions. 2024.

  \bibitem{NEURIPS2022_b125999b}
    QUARK: Controllable Text Generation with Reinforced Unlearning. 2022.

  \bibitem{madaan2023selfrefineiterativerefinementselffeedback}
    Self-Refine: Iterative Refinement with Self-Feedback. 2023.

  \bibitem{agent_llms}
    LLM-Powered Conversational Voice Assistants: Interaction Patterns, Opportunities, Challenges, and Design Guidelines. 2023.

  \bibitem{mirowski2022cowritingscreenplaystheatrescripts}
    Co-Writing Screenplays and Theatre Scripts with Language Models: An Evaluation by Industry Professionals. 2022.

  \bibitem{llm_fun_challenges_opp_and_social_impact}
    Foundation and large language models: fundamentals, challenges, opportunities, and social impacts. 2024.

  \bibitem{ollama}
    {Ollama: Get up and running with Llama 3.1, Mistral, Gemma 2, and other large language models. 2024.

  \bibitem{openai2024gpt4technicalreport}
    GPT-4 Technical Report. 2024.

  \bibitem{can_separators_improve_chain_of_thought_prompting_}
    Can Separators Improve Chain-of-Thought Prompting?. 2024.

  \bibitem{patel-etal-2021-nlp}
    Are {NLP. 2021.

  \bibitem{paul2024refinerreasoningfeedbackintermediate}
    REFINER: Reasoning Feedback on Intermediate Representations. 2024.

  \bibitem{lm_studio_-_discover_download_and_run_local_llms}
    Machine Translation with Large Language Models: Prompt Engineering for Persian, English, and Russian Directions. 2024.

  \bibitem{can_github_issues_be_solved_with_tree_of_thoughts_}
    Can Github issues be solved with Tree Of Thoughts?. 2024.

  \bibitem{can_llm_master_math_no}
    Can LLMs Master Math? Investigating Large Language Models on Math Stack Exchange. 2024.

  \bibitem{algorithm_of_thoughts_enhancing_exploration_of_ideas_in_large_language_models}
    Algorithm of Thoughts: Enhancing Exploration of Ideas in Large Language Models. 2023.

  \bibitem{small_llms_are_weak_tool_learners_a_multi_llm_agent}
    Small LLMs Are Weak Tool Learners: A Multi-LLM Agent. 2024.

  \bibitem{shinn2023reflexionlanguageagentsverbal}
    Reflexion: Language Agents with Verbal Reinforcement Learning. 2023.

  \bibitem{chain_of_thoughtlessness}
    Chain of Thoughtlessness? An Analysis of CoT in Planning. 2024.

  \bibitem{learntorepair}
    {Learning to Repair: Repairing model output errors after deployment using a dynamic memory of feedback. 2021.

  \bibitem{gemma_2024}
    Gemma. 2024.

  \bibitem{LLMs_generate_human-like_opinions}
    ChatGPT as a commenter to the news: can LLMs generate human-like opinions?. 2023.

  \bibitem{van2024hybrid}
    A hybrid intelligence method for argument mining. 2024.

  \bibitem{vatsal2024surveypromptengineeringmethods}
    A Survey of Prompt Engineering Methods in Large Language Models for Different NLP Tasks. 2024.

  \bibitem{self_consistency_improves_chain_of_thought_reasoning_in_language_models}
    Self-Consistency Improves Chain of Thought Reasoning in Language Models. 2022.

  \bibitem{wang2024describeexplainplanselect}
    Describe, Explain, Plan and Select: Interactive Planning with Large Language Models Enables Open-World Multi-Task Agents. 2024.

  \bibitem{chain_of_thought_prompting_elicits_reasoning_in_large_language_models}
    Chain-of-Thought Prompting Elicits Reasoning in Large Language Models. 2022.

  \bibitem{welleck2022generatingsequenceslearningselfcorrect}
    Generating Sequences by Learning to Self-Correct. 2022.

  \bibitem{decomosition_of_task_with_llms}
    MLDT: Multi-Level Decomposition for Complex Long-Horizon Robotic Task Planning with Open-Source Large Language Model. 2024.

  \bibitem{xie2023selfevaluationguidedbeamsearch}
    Self-Evaluation Guided Beam Search for Reasoning. 2023.

  \bibitem{xing2024designing}
    Designing heterogeneous llm agents for financial sentiment analysis. 2024.

  \bibitem{unlocking_the_potential_a_comprehensive_exploration_of_large_language_models_in_natural_language_processing}
    Unlocking the potential: A comprehensive exploration of large language models in natural language processing. 2024.

  \bibitem{generative_ai_in_the_era_of_transformers_revolutionizing_natural_language_processing_with_llms}
    Generative AI in the Era of Transformers: Revolutionizing Natural Language Processing with LLMs. 2024.

  \bibitem{large_language_models_are_contrastive_reasoners}
    Large Language Models are Contrastive Reasoners. 2024.

  \bibitem{tree_of_thoughts_deliberate_problem_solving_with_large_language_models}
    Tree of Thoughts: Deliberate Problem Solving with Large Language Models. 2023.

  \bibitem{yao2023reactsynergizingreasoningacting}
    ReAct: Synergizing Reasoning and Acting in Language Models. 2023.

  \bibitem{llm_healthcare}
    Leveraging generative AI and large Language models: a Comprehensive Roadmap for Healthcare Integration. 2023.

  \bibitem{text_Summary}
    A Systematic Survey of Text Summarization: From Statistical Methods to Large Language Models. 2024.

  \bibitem{zhang2023exploring}
    Exploring collaboration mechanisms for llm agents: A social psychology view. 2023.

  \bibitem{gaokao-math}
    Evaluating the Performance of Large Language Models on GAOKAO Benchmark. 2023.

  \bibitem{zhou2024misinformingllmsvulnerabilitieschallenges}
    Misinforming LLMs: vulnerabilities, challenges and opportunities. 2024.

  \bibitem{least_to_most_prompting_enables_complex_reasoning_in_large_language_models}
    Least-to-Most Prompting Enables Complex Reasoning in Large Language Models. 2022.

\end{thebibliography}
